Situated Conditional Reasoning

Conditionals are useful for modelling, but are not always sufficiently expressive for capturing information accurately. In this paper we make the case for a form of conditional that is situation-based. These conditionals are more expressive than classical conditionals, are general enough to be used in several application domains, and are able to distinguish, for example, between expectations and counterfactuals. Formally, they are shown to generalise the conditional setting in the style of Kraus, Lehmann, and Magidor. We show that situation-based conditionals can be described in terms of a set of rationality postulates. We then propose an intuitive semantics for these conditionals, and present a representation result which shows that our semantic construction corresponds exactly to the description in terms of postulates. With the semantics in place, we proceed to define a form of entailment for situated conditional knowledge bases, which we refer to as minimal closure. It is reminiscent of and, indeed, inspired by, the version of entailment for propositional conditional knowledge bases known as rational closure. Finally, we proceed to show that it is possible to reduce the computation of minimal closure to a series of propositional entailment and satisfiability checks. While this is also the case for rational closure, it is somewhat surprising that the result carries over to minimal closure.

==> 1stResponseLetter/AIJ-SituatedConditionals-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General expressions and commands:

\newcommand{\ie}{\mbox{i.e.}}
\newcommand{\eg}{\mbox{e.g.}}
\newcommand{\cf}{\mbox{cf.}}
\newcommand{\viz}{\mbox{viz.}}
\newcommand{\wrt}{\mbox{w.r.t.}}
\newcommand{\st}{\mbox{s.t.}}
\newcommand{\wolog}{\mbox{w.l.o.g.}}
\newcommand{\etal}{\mbox{et al}}
\newcommand{\aka}{\mbox{a.k.a.}}
\newcommand{\myskip}{\smallskip} % space interlines
\newcommand{\df}[1]{\textbf{#1}} % to emphasise defined terms in definitions
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical general expressions:

%\newcommand{\qed}{\rule{2mm}{2mm}}%{[\textsc{qed}]}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\defined}{\:\raisebox{1ex}{\scalebox{0.5}{\ensuremath{\mathrm{def}}}}\hskip-1.65ex\raisebox{-0.1ex}{\ensuremath{=}}\:}
\newcommand{\eqclass}[1]{[#1]} % equivalence class of an element
\newcommand{\assigned}{\mathrel{\mathop:}=}
\newcommand{\grammar}{\mathrel{\mathop:}\gets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environments:

%\theoremstyle{break}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
%\newtheorem{conjecture}{Conjecture}%[section]
%\newtheorem{observation}{Observation}%[section]
%\newtheorem{claim}{Claim}%[section]
%{\theorembodyfont{\upshape}
\newtheorem{example}{Example}[section]%}
%{\theoremstyle{plain}\theorembodyfont{\upshape}
%\newtheorem{remark}{Remark}%[section]%}
%\newenvironment{proof}{\noindent\textbf{Proof:}\null\hfill\null\newline}{\hfill\qed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational complexity:

\newcommand{\Ptime}{\textsc{P}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\ExpTime}{\textsc{exptime}}
\newcommand{\PSpace}{\textsc{pspace}}
\newcommand{\NPC}{\textsc{np-complete}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special sets:

% Language:
\newcommand{\Prp}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}} % the set of sentences of a language

% Theories:
\newcommand{\T}{\ensuremath{\mathcal{T}}} % a theory
\newcommand{\KB}{\ensuremath{\mathcal{KB}}} % a knowledge base

% Semantics:
\newcommand{\U}{\ensuremath{\mathcal{U}}} % set of all propositional valuations
\newcommand{\Val}{\ensuremath{\mathcal{V}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special functions and relations:

\newcommand{\id}{\ensuremath{\text{\it id}}} % identity relation
\newcommand{\atm}{\ensuremath{\text{\it atm}}} % atoms of a sentence
\newcommand{\lit}{\ensuremath{\text{\it lit}}} % literals of a sentence
\newcommand{\sig}{\ensuremath{\text{\it sig}}} % symbols of a sentence
%\newcommand{\Mod}{\ensuremath{\text{\it Mod}}} % models of a sentence
\newcommand{\Mod}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\Cn}{\ensuremath{\text{\it Cn}}} % logical consequence
\newcommand{\pImp}{\ensuremath{\text{\it PI}}} % set of prime implicates
\newcommand{\impP}{\ensuremath{\text{\it IP}}} % set of prime implicants
\newcommand{\NC}{\ensuremath{\text{\it NewCons}}} % new consequences
\newcommand{\sub}{\ensuremath{\text{\it sub}}} % subexpressions
\newcommand{\fm}[1]{\ensuremath{{\sf sent}({#1})}} % the sentence of a set of worlds

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Logical connectives and meta-logical basic definitions:

% Logical negation: \lnot, Logical conjunction: \land, Logical disjunction: \lor
\newcommand{\limp}{\rightarrow} % logical implication
\newcommand{\liff}{\leftrightarrow} % biconditional
\newcommand{\lexor}{\oplus} % exclusive or
\renewcommand{\bar}[1]{\overline{#1}} % barred literals

% Satisfaction, entailment and derivability relations:
\newcommand{\sat}{\Vdash}
\newcommand{\nsat}{\not\sat}
\newcommand{\entails}{\models}
\newcommand{\nentails}{\not\entails}
\newcommand{\entailed}{\raisebox{1.1ex}{\rotatebox{180}{$\entails$}}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\not\proves}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defeasible stuff:

% Language:
\newcommand{\dimp}{\leadsto}
\newcommand{\ndimp}{\not\dimp}
\newcommand{\twiddle}{\mathrel|\joinrel\sim}
\newcommand{\ntwiddle}{\not\twiddle}
\newcommand{\dsubs}{\:\raisebox{0.45ex}{\ensuremath{\sqsubset}}\hskip-1.7ex\raisebox{-0.6ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\ndsubs}{\not\!\!\!\dsubs}
\newcommand{\dequiv}{\:\raisebox{0.45ex}{\ensuremath{=}}\hskip-1.7ex\raisebox{-0.3ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\dforall}{\mathrel{\scalebox{0.73}{\raisebox{0.46ex}{$\bigvee$}}}%
						\hskip-1.79ex\joinrel\scalebox{0.88}{\raisebox{0.4ex}{$\sim$}}}
\newcommand*{\leftpartdexists}{%
      			\mathrel{\vcenter{\offinterlineskip
      			\vskip-0.45ex\hbox{\scalebox{0.77}{$-$}}\hbox{\scalebox{0.68}{\hskip0.12ex$\sim$}}%
						\vskip-0.23ex\hbox{\scalebox{0.77}{$-$}}}}}
\newcommand{\dexists}{\mathrel{\leftpartdexists}\hskip-.653ex\joinrel\scalebox{0.685}%
						{\raisebox{0.587ex}{|}}}
\newcommand{\typ}{\bullet}
\newcommand{\Typ}{\mathbf{T}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}

% Semantics:
\newcommand{\PI}{\ensuremath{\mathcal{P}}} % preferential DL interpretation
%\newcommand{\RI}{\ensuremath{\mathcal{R}}} % r-ordered interpretation
\newcommand{\pref}{\prec} % preference relation
\newcommand{\npref}{\not\pref}
\newcommand{\rk}{\ensuremath{\text{\it rk}}} % ranking function
\newcommand{\RM}{\mathscr{R}} % ranked model
\newcommand{\states}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\R}{\ensuremath{\text{\it Rk}}}
\newcommand{\ei}{\ensuremath{\text{\it e}}}
\newcommand{\EI}{\mathscr{E}} % epistemic interpretation
%\newcommand{\EI}{\ensuremath{\text{\it E}}} 
\newcommand{\ES}{\ensuremath{\mathcal{E}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}} % exceptionality function

% Entailment:
\newcommand{\dentails}{\mathrel|\joinrel\approx}
\newcommand{\ndentails}{\not\NMentails}
\newcommand{\dproves}{\mathrel|\joinrel\sim}
\newcommand{\ndproves}{\not\NMproves}
\newcommand{\miniment}{\entails_{m}}

\newcommand{\f}{\ensuremath{\mathtt{f}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to use in examples:

\newcommand{\avi}{\ensuremath{\mathsf{a}}}
\newcommand{\mam}{\ensuremath{\mathsf{m}}}
\newcommand{\nuc}{\ensuremath{\mathsf{n}}}
\newcommand{\vtb}{\ensuremath{\mathsf{v}}}
\newcommand{\extra}{\ensuremath{\mathsf{e}}}

\newcommand{\ce}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\bird}{\ensuremath{\mathsf{b}}}
\newcommand{\flies}{\ensuremath{\mathsf{f}}}
\newcommand{\peng}{\ensuremath{\mathsf{p}}}
\newcommand{\dodo}{\ensuremath{\mathsf{d}}}
\newcommand{\mc}{\ensuremath{\mathsf{mc}}}
\newcommand{\epeng}{\ensuremath{\mathsf{ep}}}
\newcommand{\rob}{\ensuremath{\mathsf{r}}}

\newcommand{\p}{\sf p}
\newcommand{\q}{\sf q}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colored text:

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 1stSubmissionToAIJ/AIJ-SituatedConditionals-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General expressions and commands:

\newcommand{\ie}{\mbox{i.e.}}
\newcommand{\eg}{\mbox{e.g.}}
\newcommand{\cf}{\mbox{cf.}}
\newcommand{\viz}{\mbox{viz.}}
\newcommand{\wrt}{\mbox{w.r.t.}}
\newcommand{\st}{\mbox{s.t.}}
\newcommand{\wolog}{\mbox{w.l.o.g.}}
\newcommand{\etal}{\mbox{et al}}
\newcommand{\aka}{\mbox{a.k.a.}}
\newcommand{\myskip}{\smallskip} % space interlines
\newcommand{\df}[1]{\textbf{#1}} % to emphasise defined terms in definitions
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical general expressions:

%\newcommand{\qed}{\rule{2mm}{2mm}}%{[\textsc{qed}]}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\defined}{\:\raisebox{1ex}{\scalebox{0.5}{\ensuremath{\mathrm{def}}}}\hskip-1.65ex\raisebox{-0.1ex}{\ensuremath{=}}\:}
\newcommand{\eqclass}[1]{[#1]} % equivalence class of an element
\newcommand{\assigned}{\mathrel{\mathop:}=}
\newcommand{\grammar}{\mathrel{\mathop:}\gets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environments:

%\theoremstyle{break}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
%\newtheorem{conjecture}{Conjecture}%[section]
%\newtheorem{observation}{Observation}%[section]
%\newtheorem{claim}{Claim}%[section]
%{\theorembodyfont{\upshape}
\newtheorem{example}{Example}[section]%}
%{\theoremstyle{plain}\theorembodyfont{\upshape}
%\newtheorem{remark}{Remark}%[section]%}
%\newenvironment{proof}{\noindent\textbf{Proof:}\null\hfill\null\newline}{\hfill\qed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational complexity:

\newcommand{\Ptime}{\textsc{P}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\ExpTime}{\textsc{exptime}}
\newcommand{\PSpace}{\textsc{pspace}}
\newcommand{\NPC}{\textsc{np-complete}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special sets:

% Language:
\newcommand{\Prp}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}} % the set of sentences of a language

% Theories:
\newcommand{\T}{\ensuremath{\mathcal{T}}} % a theory
\newcommand{\KB}{\ensuremath{\mathcal{KB}}} % a knowledge base

% Semantics:
\newcommand{\U}{\ensuremath{\mathcal{U}}} % set of all propositional valuations
\newcommand{\Val}{\ensuremath{\mathcal{V}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special functions and relations:

\newcommand{\id}{\ensuremath{\text{\it id}}} % identity relation
\newcommand{\atm}{\ensuremath{\text{\it atm}}} % atoms of a sentence
\newcommand{\lit}{\ensuremath{\text{\it lit}}} % literals of a sentence
\newcommand{\sig}{\ensuremath{\text{\it sig}}} % symbols of a sentence
%\newcommand{\Mod}{\ensuremath{\text{\it Mod}}} % models of a sentence
\newcommand{\Mod}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\Cn}{\ensuremath{\text{\it Cn}}} % logical consequence
\newcommand{\pImp}{\ensuremath{\text{\it PI}}} % set of prime implicates
\newcommand{\impP}{\ensuremath{\text{\it IP}}} % set of prime implicants
\newcommand{\NC}{\ensuremath{\text{\it NewCons}}} % new consequences
\newcommand{\sub}{\ensuremath{\text{\it sub}}} % subexpressions
\newcommand{\fm}[1]{\ensuremath{{\sf sent}({#1})}} % the sentence of a set of worlds

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Logical connectives and meta-logical basic definitions:

% Logical negation: \lnot, Logical conjunction: \land, Logical disjunction: \lor
\newcommand{\limp}{\rightarrow} % logical implication
\newcommand{\liff}{\leftrightarrow} % biconditional
\newcommand{\lexor}{\oplus} % exclusive or
\renewcommand{\bar}[1]{\overline{#1}} % barred literals

% Satisfaction, entailment and derivability relations:
\newcommand{\sat}{\Vdash}
\newcommand{\nsat}{\not\sat}
\newcommand{\entails}{\models}
\newcommand{\nentails}{\not\entails}
\newcommand{\entailed}{\raisebox{1.1ex}{\rotatebox{180}{$\entails$}}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\not\proves}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defeasible stuff:

% Language:
\newcommand{\dimp}{\leadsto}
\newcommand{\ndimp}{\not\dimp}
\newcommand{\twiddle}{\mathrel|\joinrel\sim}
\newcommand{\ntwiddle}{\not\twiddle}
\newcommand{\dsubs}{\:\raisebox{0.45ex}{\ensuremath{\sqsubset}}\hskip-1.7ex\raisebox{-0.6ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\ndsubs}{\not\!\!\!\dsubs}
\newcommand{\dequiv}{\:\raisebox{0.45ex}{\ensuremath{=}}\hskip-1.7ex\raisebox{-0.3ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\dforall}{\mathrel{\scalebox{0.73}{\raisebox{0.46ex}{$\bigvee$}}}%
						\hskip-1.79ex\joinrel\scalebox{0.88}{\raisebox{0.4ex}{$\sim$}}}
\newcommand*{\leftpartdexists}{%
      			\mathrel{\vcenter{\offinterlineskip
      			\vskip-0.45ex\hbox{\scalebox{0.77}{$-$}}\hbox{\scalebox{0.68}{\hskip0.12ex$\sim$}}%
						\vskip-0.23ex\hbox{\scalebox{0.77}{$-$}}}}}
\newcommand{\dexists}{\mathrel{\leftpartdexists}\hskip-.653ex\joinrel\scalebox{0.685}%
						{\raisebox{0.587ex}{|}}}
\newcommand{\typ}{\bullet}
\newcommand{\Typ}{\mathbf{T}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}

% Semantics:
\newcommand{\PI}{\ensuremath{\mathcal{P}}} % preferential DL interpretation
%\newcommand{\RI}{\ensuremath{\mathcal{R}}} % r-ordered interpretation
\newcommand{\pref}{\prec} % preference relation
\newcommand{\npref}{\not\pref}
\newcommand{\rk}{\ensuremath{\text{\it rk}}} % ranking function
\newcommand{\RM}{\mathscr{R}} % ranked model
\newcommand{\states}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\R}{\ensuremath{\text{\it Rk}}}
\newcommand{\ei}{\ensuremath{\text{\it e}}}
\newcommand{\EI}{\mathscr{E}} % epistemic interpretation
%\newcommand{\EI}{\ensuremath{\text{\it E}}} 
\newcommand{\ES}{\ensuremath{\mathcal{E}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}} % exceptionality function

% Entailment:
\newcommand{\dentails}{\mathrel|\joinrel\approx}
\newcommand{\ndentails}{\not\NMentails}
\newcommand{\dproves}{\mathrel|\joinrel\sim}
\newcommand{\ndproves}{\not\NMproves}
\newcommand{\miniment}{\entails_{m}}

\newcommand{\f}{\ensuremath{\mathtt{f}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to use in examples:

\newcommand{\avi}{\ensuremath{\mathsf{a}}}
\newcommand{\mam}{\ensuremath{\mathsf{m}}}
\newcommand{\nuc}{\ensuremath{\mathsf{n}}}
\newcommand{\vtb}{\ensuremath{\mathsf{v}}}
\newcommand{\extra}{\ensuremath{\mathsf{e}}}

\newcommand{\ce}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\bird}{\ensuremath{\mathsf{b}}}
\newcommand{\flies}{\ensuremath{\mathsf{f}}}
\newcommand{\peng}{\ensuremath{\mathsf{p}}}
\newcommand{\dodo}{\ensuremath{\mathsf{d}}}
\newcommand{\mc}{\ensuremath{\mathsf{mc}}}

\newcommand{\p}{\sf p}
\newcommand{\q}{\sf q}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colored text:

\newcommand{\red}[1]{\textcolor{red}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 2ndResponseLetter/AIJ-SituatedConditionals-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General expressions and commands:

\newcommand{\ie}{\mbox{i.e.}}
\newcommand{\eg}{\mbox{e.g.}}
\newcommand{\cf}{\mbox{cf.}}
\newcommand{\viz}{\mbox{viz.}}
\newcommand{\wrt}{\mbox{w.r.t.}}
\newcommand{\st}{\mbox{s.t.}}
\newcommand{\wolog}{\mbox{w.l.o.g.}}
\newcommand{\etal}{\mbox{et al}}
\newcommand{\aka}{\mbox{a.k.a.}}
\newcommand{\myskip}{\smallskip} % space interlines
\newcommand{\df}[1]{\textbf{#1}} % to emphasise defined terms in definitions
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical general expressions:

%\newcommand{\qed}{\rule{2mm}{2mm}}%{[\textsc{qed}]}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\defined}{\:\raisebox{1ex}{\scalebox{0.5}{\ensuremath{\mathrm{def}}}}\hskip-1.65ex\raisebox{-0.1ex}{\ensuremath{=}}\:}
\newcommand{\eqclass}[1]{[#1]} % equivalence class of an element
\newcommand{\assigned}{\mathrel{\mathop:}=}
\newcommand{\grammar}{\mathrel{\mathop:}\gets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environments:

%\theoremstyle{break}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
%\newtheorem{conjecture}{Conjecture}%[section]
%\newtheorem{observation}{Observation}%[section]
%\newtheorem{claim}{Claim}%[section]
%{\theorembodyfont{\upshape}
\newtheorem{example}{Example}[section]%}
%{\theoremstyle{plain}\theorembodyfont{\upshape}
%\newtheorem{remark}{Remark}%[section]%}
%\newenvironment{proof}{\noindent\textbf{Proof:}\null\hfill\null\newline}{\hfill\qed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational complexity:

\newcommand{\Ptime}{\textsc{P}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\ExpTime}{\textsc{exptime}}
\newcommand{\PSpace}{\textsc{pspace}}
\newcommand{\NPC}{\textsc{np-complete}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special sets:

% Language:
\newcommand{\Prp}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}} % the set of sentences of a language

% Theories:
\newcommand{\T}{\ensuremath{\mathcal{T}}} % a theory
\newcommand{\KB}{\ensuremath{\mathcal{KB}}} % a knowledge base

% Semantics:
\newcommand{\U}{\ensuremath{\mathcal{U}}} % set of all propositional valuations
\newcommand{\Val}{\ensuremath{\mathcal{V}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special functions and relations:

\newcommand{\id}{\ensuremath{\text{\it id}}} % identity relation
\newcommand{\atm}{\ensuremath{\text{\it atm}}} % atoms of a sentence
\newcommand{\lit}{\ensuremath{\text{\it lit}}} % literals of a sentence
\newcommand{\sig}{\ensuremath{\text{\it sig}}} % symbols of a sentence
%\newcommand{\Mod}{\ensuremath{\text{\it Mod}}} % models of a sentence
\newcommand{\Mod}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\Cn}{\ensuremath{\text{\it Cn}}} % logical consequence
\newcommand{\pImp}{\ensuremath{\text{\it PI}}} % set of prime implicates
\newcommand{\impP}{\ensuremath{\text{\it IP}}} % set of prime implicants
\newcommand{\NC}{\ensuremath{\text{\it NewCons}}} % new consequences
\newcommand{\sub}{\ensuremath{\text{\it sub}}} % subexpressions
\newcommand{\fm}[1]{\ensuremath{{\sf sent}({#1})}} % the sentence of a set of worlds

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Logical connectives and meta-logical basic definitions:

% Logical negation: \lnot, Logical conjunction: \land, Logical disjunction: \lor
\newcommand{\limp}{\rightarrow} % logical implication
\newcommand{\liff}{\leftrightarrow} % biconditional
\newcommand{\lexor}{\oplus} % exclusive or
\renewcommand{\bar}[1]{\overline{#1}} % barred literals

% Satisfaction, entailment and derivability relations:
\newcommand{\sat}{\Vdash}
\newcommand{\nsat}{\not\sat}
\newcommand{\entails}{\models}
\newcommand{\nentails}{\not\entails}
\newcommand{\entailed}{\raisebox{1.1ex}{\rotatebox{180}{$\entails$}}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\not\proves}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defeasible stuff:

% Language:
\newcommand{\dimp}{\leadsto}
\newcommand{\ndimp}{\not\dimp}
\newcommand{\twiddle}{\mathrel|\joinrel\sim}
\newcommand{\ntwiddle}{\not\twiddle}
\newcommand{\dsubs}{\:\raisebox{0.45ex}{\ensuremath{\sqsubset}}\hskip-1.7ex\raisebox{-0.6ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\ndsubs}{\not\!\!\!\dsubs}
\newcommand{\dequiv}{\:\raisebox{0.45ex}{\ensuremath{=}}\hskip-1.7ex\raisebox{-0.3ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\dforall}{\mathrel{\scalebox{0.73}{\raisebox{0.46ex}{$\bigvee$}}}%
						\hskip-1.79ex\joinrel\scalebox{0.88}{\raisebox{0.4ex}{$\sim$}}}
\newcommand*{\leftpartdexists}{%
      			\mathrel{\vcenter{\offinterlineskip
      			\vskip-0.45ex\hbox{\scalebox{0.77}{$-$}}\hbox{\scalebox{0.68}{\hskip0.12ex$\sim$}}%
						\vskip-0.23ex\hbox{\scalebox{0.77}{$-$}}}}}
\newcommand{\dexists}{\mathrel{\leftpartdexists}\hskip-.653ex\joinrel\scalebox{0.685}%
						{\raisebox{0.587ex}{|}}}
\newcommand{\typ}{\bullet}
\newcommand{\Typ}{\mathbf{T}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}

% Semantics:
\newcommand{\PI}{\ensuremath{\mathcal{P}}} % preferential DL interpretation
%\newcommand{\RI}{\ensuremath{\mathcal{R}}} % r-ordered interpretation
\newcommand{\pref}{\prec} % preference relation
\newcommand{\npref}{\not\pref}
\newcommand{\rk}{\ensuremath{\text{\it rk}}} % ranking function
\newcommand{\RM}{\mathscr{R}} % ranked model
\newcommand{\states}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\R}{\ensuremath{\text{\it Rk}}}
\newcommand{\ei}{\ensuremath{\text{\it e}}}
\newcommand{\EI}{\mathscr{E}} % epistemic interpretation
%\newcommand{\EI}{\ensuremath{\text{\it E}}} 
\newcommand{\ES}{\ensuremath{\mathcal{E}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}} % exceptionality function

% Entailment:
\newcommand{\dentails}{\mathrel|\joinrel\approx}
\newcommand{\ndentails}{\not\NMentails}
\newcommand{\dproves}{\mathrel|\joinrel\sim}
\newcommand{\ndproves}{\not\NMproves}
\newcommand{\miniment}{\entails_{m}}

\newcommand{\f}{\ensuremath{\mathtt{f}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to use in examples:

\newcommand{\avi}{\ensuremath{\mathsf{a}}}
\newcommand{\mam}{\ensuremath{\mathsf{m}}}
\newcommand{\nuc}{\ensuremath{\mathsf{n}}}
\newcommand{\vtb}{\ensuremath{\mathsf{v}}}
\newcommand{\extra}{\ensuremath{\mathsf{e}}}

\newcommand{\ce}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\bird}{\ensuremath{\mathsf{b}}}
\newcommand{\flies}{\ensuremath{\mathsf{f}}}
\newcommand{\peng}{\ensuremath{\mathsf{p}}}
\newcommand{\dodo}{\ensuremath{\mathsf{d}}}
\newcommand{\mc}{\ensuremath{\mathsf{mc}}}
\newcommand{\epeng}{\ensuremath{\mathsf{ep}}}
\newcommand{\rob}{\ensuremath{\mathsf{r}}}

\newcommand{\p}{\sf p}
\newcommand{\q}{\sf q}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colored text:

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 2ndSubmissionToAIJ/AIJ-SituatedConditionals-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General expressions and commands:

\newcommand{\ie}{\mbox{i.e.}}
\newcommand{\eg}{\mbox{e.g.}}
\newcommand{\cf}{\mbox{cf.}}
\newcommand{\viz}{\mbox{viz.}}
\newcommand{\wrt}{\mbox{w.r.t.}}
\newcommand{\st}{\mbox{s.t.}}
\newcommand{\wolog}{\mbox{w.l.o.g.}}
\newcommand{\etal}{\mbox{et al}}
\newcommand{\aka}{\mbox{a.k.a.}}
\newcommand{\myskip}{\smallskip} % space interlines
\newcommand{\df}[1]{\textbf{#1}} % to emphasise defined terms in definitions
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical general expressions:

%\newcommand{\qed}{\rule{2mm}{2mm}}%{[\textsc{qed}]}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\defined}{\:\raisebox{1ex}{\scalebox{0.5}{\ensuremath{\mathrm{def}}}}\hskip-1.65ex\raisebox{-0.1ex}{\ensuremath{=}}\:}
\newcommand{\eqclass}[1]{[#1]} % equivalence class of an element
\newcommand{\assigned}{\mathrel{\mathop:}=}
\newcommand{\grammar}{\mathrel{\mathop:}\gets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem-like environments:

%\theoremstyle{break}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
%\newtheorem{conjecture}{Conjecture}%[section]
%\newtheorem{observation}{Observation}%[section]
%\newtheorem{claim}{Claim}%[section]
%{\theorembodyfont{\upshape}
\newtheorem{example}{Example}[section]%}
%{\theoremstyle{plain}\theorembodyfont{\upshape}
%\newtheorem{remark}{Remark}%[section]%}
%\newenvironment{proof}{\noindent\textbf{Proof:}\null\hfill\null\newline}{\hfill\qed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational complexity:

\newcommand{\Ptime}{\textsc{P}}
\newcommand{\NP}{\textsc{NP}}
\newcommand{\ExpTime}{\textsc{exptime}}
\newcommand{\PSpace}{\textsc{pspace}}
\newcommand{\NPC}{\textsc{np-complete}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special sets:

% Language:
\newcommand{\Prp}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}} % the set of sentences of a language

% Theories:
\newcommand{\T}{\ensuremath{\mathcal{T}}} % a theory
\newcommand{\KB}{\ensuremath{\mathcal{KB}}} % a knowledge base

% Semantics:
\newcommand{\U}{\ensuremath{\mathcal{U}}} % set of all propositional valuations
\newcommand{\Val}{\ensuremath{\mathcal{V}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special functions and relations:

\newcommand{\id}{\ensuremath{\text{\it id}}} % identity relation
\newcommand{\atm}{\ensuremath{\text{\it atm}}} % atoms of a sentence
\newcommand{\lit}{\ensuremath{\text{\it lit}}} % literals of a sentence
\newcommand{\sig}{\ensuremath{\text{\it sig}}} % symbols of a sentence
%\newcommand{\Mod}{\ensuremath{\text{\it Mod}}} % models of a sentence
\newcommand{\Mod}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\Cn}{\ensuremath{\text{\it Cn}}} % logical consequence
\newcommand{\pImp}{\ensuremath{\text{\it PI}}} % set of prime implicates
\newcommand{\impP}{\ensuremath{\text{\it IP}}} % set of prime implicants
\newcommand{\NC}{\ensuremath{\text{\it NewCons}}} % new consequences
\newcommand{\sub}{\ensuremath{\text{\it sub}}} % subexpressions
\newcommand{\fm}[1]{\ensuremath{{\sf sent}({#1})}} % the sentence of a set of worlds

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Logical connectives and meta-logical basic definitions:

% Logical negation: \lnot, Logical conjunction: \land, Logical disjunction: \lor
\newcommand{\limp}{\rightarrow} % logical implication
\newcommand{\liff}{\leftrightarrow} % biconditional
\newcommand{\lexor}{\oplus} % exclusive or
\renewcommand{\bar}[1]{\overline{#1}} % barred literals

% Satisfaction, entailment and derivability relations:
\newcommand{\sat}{\Vdash}
\newcommand{\nsat}{\not\sat}
\newcommand{\entails}{\models}
\newcommand{\nentails}{\not\entails}
\newcommand{\entailed}{\raisebox{1.1ex}{\rotatebox{180}{$\entails$}}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\not\proves}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defeasible stuff:

% Language:
\newcommand{\dimp}{\leadsto}
\newcommand{\ndimp}{\not\dimp}
\newcommand{\twiddle}{\mathrel|\joinrel\sim}
\newcommand{\ntwiddle}{\not\twiddle}
\newcommand{\dsubs}{\:\raisebox{0.45ex}{\ensuremath{\sqsubset}}\hskip-1.7ex\raisebox{-0.6ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\ndsubs}{\not\!\!\!\dsubs}
\newcommand{\dequiv}{\:\raisebox{0.45ex}{\ensuremath{=}}\hskip-1.7ex\raisebox{-0.3ex}{\scalebox{0.9}{\ensuremath{\sim}}}\:}
\newcommand{\dforall}{\mathrel{\scalebox{0.73}{\raisebox{0.46ex}{$\bigvee$}}}%
						\hskip-1.79ex\joinrel\scalebox{0.88}{\raisebox{0.4ex}{$\sim$}}}
\newcommand*{\leftpartdexists}{%
      			\mathrel{\vcenter{\offinterlineskip
      			\vskip-0.45ex\hbox{\scalebox{0.77}{$-$}}\hbox{\scalebox{0.68}{\hskip0.12ex$\sim$}}%
						\vskip-0.23ex\hbox{\scalebox{0.77}{$-$}}}}}
\newcommand{\dexists}{\mathrel{\leftpartdexists}\hskip-.653ex\joinrel\scalebox{0.685}%
						{\raisebox{0.587ex}{|}}}
\newcommand{\typ}{\bullet}
\newcommand{\Typ}{\mathbf{T}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}

% Semantics:
\newcommand{\PI}{\ensuremath{\mathcal{P}}} % preferential DL interpretation
%\newcommand{\RI}{\ensuremath{\mathcal{R}}} % r-ordered interpretation
\newcommand{\pref}{\prec} % preference relation
\newcommand{\npref}{\not\pref}
\newcommand{\rk}{\ensuremath{\text{\it rk}}} % ranking function
\newcommand{\RM}{\mathscr{R}} % ranked model
\newcommand{\states}[1]{\llbracket#1\rrbracket} % requires package stmaryrd
\newcommand{\R}{\ensuremath{\text{\it Rk}}}
\newcommand{\ei}{\ensuremath{\text{\it e}}}
\newcommand{\EI}{\mathscr{E}} % epistemic interpretation
%\newcommand{\EI}{\ensuremath{\text{\it E}}} 
\newcommand{\ES}{\ensuremath{\mathcal{E}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}} % exceptionality function

% Entailment:
\newcommand{\dentails}{\mathrel|\joinrel\approx}
\newcommand{\ndentails}{\not\NMentails}
\newcommand{\dproves}{\mathrel|\joinrel\sim}
\newcommand{\ndproves}{\not\NMproves}
\newcommand{\miniment}{\entails_{m}}

\newcommand{\f}{\ensuremath{\mathtt{f}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to use in examples:

\newcommand{\avi}{\ensuremath{\mathsf{a}}}
\newcommand{\mam}{\ensuremath{\mathsf{m}}}
\newcommand{\nuc}{\ensuremath{\mathsf{n}}}
\newcommand{\vtb}{\ensuremath{\mathsf{v}}}
\newcommand{\extra}{\ensuremath{\mathsf{e}}}

\newcommand{\ce}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\bird}{\ensuremath{\mathsf{b}}}
\newcommand{\flies}{\ensuremath{\mathsf{f}}}
\newcommand{\peng}{\ensuremath{\mathsf{p}}}
\newcommand{\dodo}{\ensuremath{\mathsf{d}}}
\newcommand{\mc}{\ensuremath{\mathsf{mc}}}
\newcommand{\epeng}{\ensuremath{\mathsf{ep}}}
\newcommand{\rob}{\ensuremath{\mathsf{r}}}

\newcommand{\p}{\sf p}
\newcommand{\q}{\sf q}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colored text:

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End macro definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Rebuttal <==
1. Author Response
Thank you to all reviewers for constructive comments. We'll fix the typos pointed out, rephrase matters as suggested, and add the indicated bibliographic references. See below for responses to other comments and questions.

- Reviewer 2 

Question: Can you provide at least one more practically-oriented motivating example?

We opted for the dodo example since it’s representative and easy to follow, but there are more practically-oriented scenarios. E.g., Bob knows that the Kitchen has been cleaned (\neg CK |~_{\top} \bot), and has a series of (defeasible) expectations: the pan is clean (Cl) and positioned in Cupboard1 (C1) (\top |~_{\top} Cl and \top |~_{\top} C1), but if the pan is in Cupboard2 (C2) he will need a stool (St) to reach the pan (C2 |~_{\top} St). We can model Bob’s expectations about counterfactual situations. E.g., if the kitchen has not been cleaned he will find the pan in the sink (\top|~_{\neg CK} Si) and it will be dirty (\top|~_{\neg CK} \neg Cl). The conditionals can be used to change his expectations in case he needs to revise information (e.g., he discovers the kitchen has not been cleaned)


Question: Can you explain in a more convincing way the advantage of your formalism over other similar ones? 

Counterfactual reasoning in AI has relevance in many domains: causal reasoning, planning, explanations and XAI (see, e.g., Byrne, Counterfactuals in Explainable Artificial Intelligence, IJCAI 2019). The same holds for modelling expectations and defeasible reasoning, considering the ample use of non-monotonic reasoning in KR. Our approach has a role in modelling reasoning for domains in which both expectations and counterfactuals are needed.


- Reviewer 3

Comment: The only major problem is that in Definition 12, fml is not defined

fml was inadvertently commented out. fml(X) represents any formula A where X is the set of models of A. Of course we will add the formal definition back in the paper.


Comment: Definition 4: I did not immediately get the connection between the second part of Definition 4 (every minimal plausible \gamma-model is a not \alpha-model) with the explanation below it (“if the On the other hand if the context γ is not compatible with the plausible part of E (that is, all models of γ have an infinite rank) then α |∼ γ β holds if the most typical implausible (but possible) models of α ∧ γ are also models of β.”). This should be explained better.

We agree that the current phrasing of definition 4 may obscure the meaning (in fact, it contained a typo in the definition [[alpha]]_E: please see our response to reviewer 6 below). We intend to replace it with the following equivalent definition:

alpha |~_gamma beta iff 
the minimal (alpha & gamma)-models in U^f_E are beta-models whenever there are gamma-models in U^f_E;
the minimal (alpha & gamma)-models in U^\infty_E are beta-models, otherwise.  
We believe this phrasing of the definition will clear up any confusion. 


Comment: As far as I can see, Ext and SupExp imply Inc.

Correct. We feel that it is useful to mention Inc, but we’ll rephrase matters to make it clear that it follows from Ext and SupExp. 

Comment: Sentence above definition 11: should this be E2(w)\not\preceq E1(w)?

Correct. 


Question: Example 2: why is penguins are birds modelled as p&-b|~ \bot and not as p|~b?

It represents “penguins are birds” (as opposed to “penguins are usually birds”). As pointed out one paragraph above Theorem 1, a classical statement alpha can be represented as ~alpha |~ \bot. Hence, p&~b |~ \bot, which is equivalent to ~(p->b) |~ \bot, represents the classical statement p->b. 

Having pointed that out, the reviewer’s remark has made us realise that it will aid with readability to rather replace p&~b |~ \bot in Example 2 with p -> b. 


- Reviewer 4

Comment: The significance of the approach could be made clearer, e.g., by providing a realistic application scenario.

See our response to reviewer 2


Comment: p. 2, right column, l. -18: The example knowledge base contains a formula which is not given in the form of a defeasible conditional.

One paragraph above Theorem 1 we point out that we sometimes abbreviate ~alpha |~ \bot as alpha. This is one such a case: we take p -> b to abbreviate ~(p -> b) |~ \bot.


Comment: p. 4, left column: The intuitive explanation of Definition 4 given after the definition does not fully correspond to Definition 4. Please check and rephrase.

There is a typo in the definition (see the response to Remark 1 from Reviewer 6). Please check also our response to reviewer 3 about Def. 4.


Comment: p. 5, Theorem 3: At least a proof sketch should be given here.

We added the full proof in the appendix due to space considerations. 

Comment: p. 7, right column, ll 3 -- 6: There seems to be something wrong here:

We assume the reviewer means page 6.

l. 3: You probably want to have \prec_{\cal K} here instead of \preceq_{\cal K}.

Correct

l. 6: You probably want to have \prec here instead of \preceq.

Correct


Comment: p. 7, Def. 12: This definition is incomplete, You did not define what fml(...) stands for.

See response to reviewer 3 above  


Comment: p. 7, Prop. 4 and 5: At least a proof sketch should be given here.

We added the full proofs in the appendix due to space considerations


- Reviewer 6 

Main remark: 

Definition 4 does not give us that p |~_{T} \bot. According to the definition, p |~_{T} \bot iff (i) [[p]]_E subseteq [[\bot]] or (ii) \emptyset \neq [[T]]^f_E \subseteq [[~p]]. For (i), note that, [[p]]_E is not a subset of the emptyset (there is a model of p with rank <f,1>. For (ii), note that [[T]]^f_E is not a subset of [[~p]]: it contains two models of p (with ranks <f,1> and <f,2>). Since neither (i) nor (ii) is satisfied, it follows that it is not the case that p |~_{T} \bot is satisfied in E.  

About Def. 4, please check also the response to Reviewer 3: with the typo in the definition of [[alpha]]_E fixed (see response to the comment directly below), Def. 4 is correct, but we plan to change it with an equivalent definition, more immediately understandable. The results and their proofs (in the appendix) do not need to be changed.


Remark 1: 

Correct. To be more precise, the last bit of the definition of [[alpha]]_E should be “for all v \in [[alpha]] \cap U^{\infty}_E” and not “for all v \in [[alpha]]”. This is a typo that crept in.  


Remark 2: 

We agree. This property you suggest holds for FCCs.


Remark 6:

See our response regarding the set [[alpha]]_E. With the typo fixed, this remark holds. 


Remark 6 continued: For the same reason the claim (page 6, column 1) "It is easy to see that R and E^R are equivalent w.r.t. the satisfaction of defeasible conditionals." is false. Note that this claim is used in proving that the minimal model (Definition 12) is a model of the CC base.

See our response regarding the set [[alpha]]_E. With the typo fixed, this remark holds and it does not affect the proof that the minimal model is a model of the CC base. 


Remark 8: 

See response to reviewer 3


Question: What do you think about my main remark?

See response to that above. 

Question: What do you think about my remark number 6?

See response to that above. 
